Learning Long-Term Reward Redistribution via Randomized Return Decomposition

Many practical applications of reinforcement learning require agents to learn from sparse and delayed rewards. It challenges the ability of agents to attribute their actions to future outcomes. In this paper, we consider the problem formulation of episodic reinforcement learning with trajectory feedback. It refers to an extreme delay of reward signals, in which the agent can only obtain one reward signal at the end of each trajectory. A popular paradigm for this problem setting is learning with a designed auxiliary dense reward function, namely proxy reward, instead of sparse environmental signals. Based on this framework, this paper proposes a novel reward redistribution algorithm, randomized return decomposition (RRD), to learn a proxy reward function for episodic reinforcement learning. We establish a surrogate problem by Monte-Carlo sampling that scales up least-squares-based reward redistribution to long-horizon problems. We analyze our surrogate loss function by connection with existing methods in the literature, which illustrates the algorithmic properties of our approach. In experiments, we extensively evaluate our proposed method on a variety of benchmark tasks with episodic rewards and demonstrate substantial improvement over baseline algorithms.

==> 3_method-old.tex <==
\section{Reward Redistribution via Randomized Return Decomposition}

In this section, we present a novel approach to redistributing episodic rewards. To serve intuitions, we start the discussions with a simplified setting in which we assume the existence of an underlying Markovian reward function $\widehat R(s,a)$ that approximates the episodic rewards by
\begin{align} \label{eq:sum-decomposable_episodic_reward}
\text{(sum-decomposable episodic reward)} \qquad\quad R_{\text{ep}}(\tau) \approx \widehat R_{\text{ep}}(\tau) =  \sum_{t=0}^{T-1}\widehat R(s_t,a_t), \qquad\qquad\quad~
\end{align}
where $R_{\text{ep}}(\tau)$ denotes the environmental episodic reward, and $\widehat R_{\text{ep}}(\tau)$ denotes the underlying sum-decomposable reward function. This structure is commonly considered by both theoretical \citep{efroni2021reinforcement} and empirical studies \citep{liu2019sequence} in the prior literature. In this setting, the reward redistribution can be constructed by \textit{return decomposition}, i.e., decomposing the trajectory feedback $R_{\text{ep}(\tau)}$ to the underlying Markovian rewards $\widehat R(s,a)$. In practice, \citet{liu2019sequence} trains a parameterized proxy reward function $\widehat R_\theta$ by optimizing the following loss function:
\begin{align} \label{eq:return_decomposition_loss}
	\mathcal{L}_{\text{RD}}(\theta) = \mathop{\mathbb{E}}_{\tau\sim\mathcal{D}} \left[\biggl(R_{\text{ep}}(\tau)-\sum_{t=0}^{T-1}\widehat R_{\theta}(s_t, a_t)\biggr)^2\right],
\end{align}
where $\mathcal{D}$ denotes the experience dataset collected by the agent. Assuming the above loss function is properly optimized, the least-squares estimation $\widehat R_{\theta}(s,a)$ is expected to asymptotically concentrate near the ground-truth underlying rewards $\widehat R(s,a)$.

\paragraph{Scalability Limitation of Return Decomposition.}
One major limitation of the return decomposition method stated in Eq.~\eqref{eq:return_decomposition_loss} is its scalability with respect to the trajectory length $T$.

\boxed{TODO} an example

\subsection{Concentratability of Dense Reward Signals}

Our reward redistribution mechanism is motivated by a common belief that reinforcement learning algorithms prefer \textit{dense} reward signals in practice \citep{zheng2018learning, jiang2019hierarchical, gangwani2019learning, gangwani2020learning, okudo2021reward}. To ensure the learned proxy rewards are dense signals, we propose to conduct a structural constraint on the redistributed rewards. Formally, we note that a \textit{dense} reward function satisfies the \textit{concentratability} property as the following statement:
\begin{definition}[Concentratability]
	Let $\widehat R(s,a)$ denote a dense reward function. The episodic return $\widehat R_{\text{ep}}(\tau)=\sum_{t=0}^{T-1}\widehat R(s_t,a_t)$ can be properly estimated by randomly sampling a subset of state-action pairs $\{(s_t,a_t)\}\subset\tau$ from the agent trajectory. i.e.,
	\begin{align} \label{eq:concentratability}
		R_{\text{ep}}(\tau) = \sum_{t=0}^{T-1}\widehat R(s_t,a_t) \approx \frac{T}{|\mathcal{I}|}\sum_{t\in\mathcal{I}}\widehat R(s_t, a_t),
	\end{align}
	where $\mathcal{I}\subseteq [T]$ denotes a random subset of timestep indices with size $|\mathcal{I}|\ll T$.
\end{definition}

\subsection{Randomized Return Decomposition Loss}

We propose to leverage the concentratability property as a structural constraint for reward redistribution. The objective function of our approach is formulated by the \textit{randomized return decomposition} loss $\mathcal{L}_{\text{Rand-RD}}(\theta)$ stated in Eq.~\eqref{eq:Rand-RD_loss}, in which the parameterized proxy reward function $\widehat R_\theta$ is trained to predict the episodic return $R_{\text{ep}}(\tau)$ given a random subsequence of the agent trajectory.
\begin{align} \label{eq:Rand-RD_loss}
	\mathcal{L}_{\text{Rand-RD}}(\theta) = \mathop{\mathbb{E}}_{\tau\sim\mathcal{D}} \left[\mathop{\mathbb{E}}_{\mathcal{I}\sim\rho(T)}\left[\biggl(R_{\text{ep}}(\tau)-\frac{T}{|\mathcal{I}|}\sum_{t\in\mathcal{I}}\widehat R_{\theta}(s_t, a_t)\biggr)^2\right]\right],
\end{align}
where $\rho(T)$ denotes the sampling distribution of subsequence $\mathcal{I}$.

\subsection{Algorithm Analysis}

\begin{restatable}[test]{theorem}{SurrogateBound}
	\begin{align*}
		\mathcal{L}_{\text{Rand-RD}}(\theta) = \mathcal{L}_{\text{RD}}(\theta) + \mathop{\mathbb{E}}_{\tau\sim\mathcal{D}} \Biggl[\mathop{\text{Var}}_{\mathcal{I}\sim\rho(T)}\left[\frac{T}{|\mathcal{I}|}\sum_{t\in\mathcal{I}}\widehat R_{\theta}(s_t, a_t)\right]\Biggr] \geq \mathcal{L}_{\text{RD}}(\theta)
	\end{align*}
\end{restatable}

